Does Your Model Classify Entities Reasonably? Diagnosing and Mitigating Spurious Correlations in Entity Typing

Entity typing aims at predicting one or more words that describe the type(s) of a specific mention in a sentence. Due to shortcuts from surface patterns to annotated entity labels and biased training, existing entity typing models are subject to the problem of spurious correlations. To comprehensively investigate the faithfulness and reliability of entity typing methods, we first systematically define distinct kinds of model biases that are reflected mainly from spurious correlations. Particularly, we identify six types of existing model biases, including mention-context bias, lexical overlapping bias, named entity bias, pronoun bias, dependency bias, and overgeneralization bias. To mitigate model biases, we then introduce a counterfactual data augmentation method. By augmenting the original training set with their debiased counterparts, models are forced to fully comprehend sentences and discover the fundamental cues for entity typing, rather than relying on spurious correlations for shortcuts. Experimental results on the UFET dataset show our counterfactual data augmentation approach helps improve generalization of different entity typing models with consistently better performance on both the original and debiased test sets.

==> 2_problem.tex <==
\subsection{Problem Definition}
Given a sentence with $s$ an entity mention $e\in s$, the \emph{entity typing} task aims at predicting one or more words or phrases $T$ from the label space $L$ that describe the type(s) of $e$.

To benefit the downstream context-sensitive tasks with identified entity types, we require that the selected entity type $T$ should be context sensitive. Take the 1st sample demonstrated in~\Cref{fig:spurious_correlations} as an instance: in ``Last week I stayed in Treasure Island for two nights when visiting Las Vegas,'' Treasure Island should be typed as ``hotel'' and ``resort'', rather than ``island'' or ``land''.

The definition of the label space $L$ varies across literature: some focused on predicting free-form words (e.g., place, hotel, etc)~\cite{ling2012fine,choi-etal-2018-ultra}, while the others aimed at predicting labels organized into a type hierarchy (e.g., /location/hotel) to allow domain knowledge incorporation and ensure label consistency~\cite{gillick2014context}. Considering the unclear hierarchy in the studied large-scale label space, we adopting the free-form types without ontologies in this work. Nevertheless, strategies to diagnose and mitigate spurious correlations proposed in this paper should apply to tasks on hierarchical label space as well.

==> 3_method_old.tex <==
\section{Method}
\nan{S,T meaning}
\begin{table*}[h!]
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lll@{}}
\toprule
Bias Types                                                                                                                                                               & Masked Fill-in Instances                                                                                                                                                                                                                                                                                                                                                                     & Entity Typing Instances                                   \\ \midrule\midrule
\begin{tabular}[t]{@{}ll}\textbf{Mention-Context}: \\ Models overly rely\\ on surface patterns \\ of mentions to predict\end{tabular}                                           & \begin{tabular}[t]{@{}ll}\hypertarget{s1}{\textbf{\textcolor{red}{S1}}}: \underline{\textbf{\emph {fire}}} is a type of \emph{\textless{}mask\textgreater{}}.\\ \textbf{\emph{RoBERTa}}: \emph{energy, heat, explosion, fire, gas}\\\\\hypertarget{s2}{\textbf{\textcolor{red}{S2}}}: \underline{\textbf{\emph{the war}}} is a type of \emph{<mask>}.\\\textbf{True labels}: \emph{war, battle, conflict}\\\textbf{\emph{RoBERTa}}: \emph{war, battle, conflict, violence,}\\\emph{warfare}\end{tabular}           & \begin{tabular}[t]{@{}ll}\hypertarget{t1}{\textbf{\textcolor{blue}{T1}}}: A teacher who survived the school shooting has said he will never\\forgive the police for taking over an hour to enter his classroom after \\the gunman first opened \underline{\textbf{\emph {fire}}} . \\ \textbf{True labels}: \emph{injury, shooting, event, violence}\\ \textbf{\emph{MLMET}}: \emph{event, object, fire} (F1: 0.285)\\ \cmidrule(r){2-3} \hypertarget{t2}{\textbf{\textcolor{blue}{T2}}}: \underline{\textbf{\emph {fire}}}\\ \textbf{\emph{MLMET}}: \emph{object, fire} (F1: 0.0)\end{tabular}\\\midrule\midrule

\begin{tabular}[t]{@{}ll}\textbf{Lexical Overlapping}:\\ Models predict labels that \\ have high lexical overlapping \\ with mention words\end{tabular}                         & \begin{tabular}[t]{@{}ll}\hypertarget{s3}{\textbf{\textcolor{red}{S3}}}: \underline{\textbf{\emph {Next twenty-four hour period}}} , after \\ the Slovaks captured Rymanow Zdroj \\ and the Germans seized Krosno , the \\ Brigade was ordered to withdraw to \\ Sanok and leave Dukla . \underline{\textbf{\emph {Next}}} \\ \underline{\textbf{\emph {twenty-four hour period}}} is a type \\ of \emph{\textless{}mask\textgreater{}}.\\ \textbf{\emph{RoBERTa}}: \emph{confusion, retreat, ambush,} \\                   \emph{battle, timeline}\end{tabular} & \begin{tabular}[t]{@{}ll}\hypertarget{t3}{\textbf{\textcolor{blue}{T3}}}: \underline{\textbf{\emph {Next day}}} , after the Slovaks captured Rymanow Zdroj and the \\ Germans seized Krosno , the Brigade was ordered to withdraw to \\ Sanok and leave Dukla .\\ \textbf{True labels}: \emph{day, time, event, date, year}\\ \textbf{\emph{MLMET}}: \emph{day, time, date} (F1: 0.749)\\ \cmidrule(r){2-3} \hypertarget{t4}{\textbf{\textcolor{green}{T4}}}: \underline{\textbf{\emph {Next twenty-four hour period}}} , after the Slovaks captured \\ Rymanow Zdroj and the Germans seized Krosno , the Brigade \\ was ordered to withdraw to Sanok and leave Dukla .\\ \textbf{\emph{MLMET}}: \emph{time, hour, period} (F1: 0.25)\end{tabular}\\\midrule\midrule
\begin{tabular}[t]{@{}ll}\textbf{Named Entity}: \\ Models leverage shortcuts \\ between recognized named \\ entities and annotated \\ labels regardless of content\end{tabular} & \begin{tabular}[t]{@{}ll}\hypertarget{s4}{\textbf{\textcolor{red}{S4}}}: The person \underline{\textbf{\emph {Benjamin Netanyahu}}} is a \\type of \emph{\textless{}mask\textgreater{}}.\\ \textbf{\emph{RoBERTa}}: \emph{politician, person, character,} \\                   \emph{personality, man}
% \end{tabular}
\\ \\ \hypertarget{s5}{\textbf{\textcolor{red}{S5}}}: The person \underline{\textbf{\emph{Jintara Poonlarp}}} is a type\\ of \emph{\textless{}mask\textgreater{}}.\\ \textbf{\emph{RoBERTa}}: \emph{person, human, woman, } \\                    \emph{personality, character}\end{tabular} 
& \begin{tabular}[t]{@{}ll}\hypertarget{t5}{\textbf{\textcolor{blue}{T5}}}: \underline{\textbf{\emph{Benjamin Netanyahu}}} asserted that Amin al-Husseini had been\\ one of the masterminds of the Holocaust .\\ \textbf{True labels}: \emph{politician, leader, person}\\ \textbf{\emph{MLMET}}: \emph{politician, leader, person} (F1: 1.0)\\ \cmidrule(r){2-3}\hypertarget{t6}{\textbf{\textcolor{green}{T6}}}: \underline{\textbf{\emph{Jintara Poonlarp}}} asserted that Amin al-Husseini had been\\ one of the masterminds of the Holocaust .\\ \textbf{\emph{MLMET}}: \emph{person, scholar, writer} (F1: 0.333)\end{tabular} \\\midrule\midrule
\begin{tabular}[t]{@{}ll}\textbf{Pronoun}:\\ Models are subject to biased \\ training to type frequent \\ pronouns, but fail to type \\ based on real names\end{tabular}        & \begin{tabular}[t]{@{}ll}\hypertarget{s6}{\textbf{\textcolor{red}{S6}}}: \underline{\textbf{\emph{Judith}}} other film credits include `` The\\ Four Feathers , '' ``  Dr. T \& amp ; the \\Women '' and `` 200 Cigarettes . '' \underline{\textbf{\emph {Judith}}}  is \\a type of \emph{\textless{}mask\textgreater{}}.\\ \textbf{\emph{RoBERTa}}: \emph{bird, cat, vampire, rabbit, dog}\end{tabular}                                                                                                                                    & \begin{tabular}[t]{@{}ll}\hypertarget{t7}{\textbf{\textcolor{blue}{T7}}}: \underline{\textbf{\emph{Her}}} other film credits include `` The Four Feathers , '' ``  Dr. T \&\\ amp ; the Women '' and `` 200 Cigarettes . ''\\ \textbf{True labels}: \emph{woman, performer, adult, female, entertainer, person,} \\                     \emph{actress}\\ \textbf{\emph{MLMET}}: \emph{woman, female, actress, person, artist} (F1: 0.666)\\ \cmidrule(r){2-3} \hypertarget{t8}{\textbf{\textcolor{green}{T8}}}: \underline{\textbf{\emph{Judith}}} other film credits include `` The Four Feathers , '' ``  Dr. T \&\\ amp ; the Women '' and `` 200 Cigarettes . ''\\ \textbf{\emph{MLMET}}: \emph{person} (F1: 0.25)\end{tabular}\\ \bottomrule
\end{tabular}%
}
\caption{Entity typing instances with content-based biases recognized by RoBERTa-large~\cite{liu2019roberta}. To reflect the shortcuts exploited by entity typing models (\Cref{sec:spurious_correlation_definition}), we list the sentences, labels and predictions from one of the SOTA models \emph{MLMET} in \textcolor{blue}{T1}, \textcolor{blue}{T2}, \textcolor{blue}{T3}, \textcolor{blue}{T5} and \textcolor{blue}{T7}. To quantify models' leverage of spurious correlations (\Cref{sec:diagnosing_et_models}), we show the constructed masked fill-in task to query the mention type from the PLM with some necessary context from \textcolor{red}{S1} to \textcolor{red}{S6}. To mitigate spurious correlations (\Cref{sec:mitigating_spurious_correlations}), we show the proposed counterfactual data augmentation where the shortcuts disappear and the model fails in \textcolor{green}{T4}, \textcolor{green}{T6} and \textcolor{green}{T8}. We underline the \underline{\textbf{\emph{mention span}}} in italic boldface and record the macro f1 score after predictions in this and following demonstrations.}
\label{tab:bias_example_I}
\end{table*}
\begin{table*}[t!]
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lll@{}}
\toprule
Bias Type                                                                                                                                                                                                         & Analyses                                                                                                                                                                                                                                                                                         & Entity Typing Instances\\ \midrule\midrule
\begin{tabular}[t]{@{}ll}\textbf{Dependency}:\\ Models fail to capture the \\ syntactic structure and \\ make type predictions \\ focusing on other \\ components rather \\ than the dependency \\ headword\end{tabular} & \begin{tabular}[t]{@{}ll}\text{Mention}:  \hypertarget{s6}{\textbf{\textcolor{green}{S6} Dependency Parsing}}: \\ 
\underline{
token | text | head text}\\ 1st\quad\quad whale  \quad anatomy\\ 2nd \quad  anatomy\quad anatomy\end{tabular}                                                                                           & \begin{tabular}[t]{@{}ll}\hypertarget{t9}{\textbf{\textcolor{blue}{T9}}}: Dubois contributed an article on \underline{\textbf{\emph{whale anatomy}}} to a book by the Dutch zoologist ,  Max \\Wsubjecteber , and , inspired by the fresh discovery of new Neanderthal fossils at  the Belgian\\ town of Spy , he spent his vacation fossil hunting in the vicinity of his birthplace .\\ \textbf{True labels}: \emph{subject, topic}\\ \textbf{\emph{MLMET}}: \emph{object, animal} (F1: 0.0)\\\cmidrule(r){2-3} \hypertarget{t10}{\textbf{\textcolor{green}{T10}}}: Dubois contributed an article on \underline{\textbf{\emph{anatomy}}} to a book by the Dutch zoologist ,  Max \\Wsubjecteber , and , inspired by the fresh discovery of new Neanderthal fossils at the  Belgian\\ town of Spy, he spent his vacation fossil hunting in the vicinity of his birthplace .\\ \textbf{\emph{MLMET}}: \emph{object, concept, subject} (F1: 0.4)\end{tabular} \\\midrule\midrule
\begin{tabular}[t]{@{}ll}\textbf{Overgeneralization}:\\ Models suffer from \\ biased training \\ due to extreme class \\ imbalance\end{tabular}                                                                          & \begin{tabular}[t]{@{}ll}\textbf{\textcolor{blue}{Statistics}}:\\\textbf{Counts of Coarse Types}:\\\emph{person}: 824, \emph{event}: 181\\\textbf{Counts of Ultra-fine Types}:\\ \emph{concept}: 68, \emph{activity}: 23,\\ \emph{trouble}: 8, \emph{difficulty}: 6,\\ \emph{problem}: 5, \emph{misconduct}: 1,\\\emph{use}: 1, \emph{abuse}: 0\\ \emph{behavior}: 0, \emph{wrongdoing}: 0\end{tabular} & \begin{tabular}[t]{@{}ll}\hypertarget{t11}{\textbf{\textcolor{blue}{T11}}}: \underline{\textbf{\emph{Many nineteenth-century individualist anarchists ,}}} including Benjamin Tucker , rejected\\ the anarcho-capitalist Lockean position in favour of the anarchist position of '' occupancy and \\use '' -LRB- or '' possession '' , to use Proudhon 's term -RRB- , particularly in land .\\ \textbf{True labels}: \emph{person}\\ \textbf{\emph{MLMET}}: \emph{person} (F1: 1.0)\\\cmidrule(r){2-3}
\hypertarget{t12}{\textbf{\textcolor{blue}{T12}}}: In a letter , the exchange said its investigations had turned up `` no evidence  of \underline{\textbf{\emph{abusive}}}\\ \underline{\textbf{\emph{behavior}}} . ''\\ \textbf{True labels}: \emph{behavior, wrongdoing, difficulty, misconduct, trouble, use, activity, problem, } \\ \emph{concept, abuse}\\ \textbf{\emph{MLMET}}: \emph{behavior, event} (F1: 0.166) \\\cmidrule(r){2-3}
\hypertarget{t13}{\textbf{\textcolor{red}{T13}}}: <NULL Input>\\
\textbf{\emph{MLMET}}:\emph{person }(prob=0.992)\end{tabular}
\\ \bottomrule
\end{tabular}%
}
\caption{Entity typing instances from \emph{UFET} test set with biases detected based on statistical analyses. To discover shortcuts utilized by entity typing models (\Cref{sec:spurious_correlation_definition}), we show one \emph{Dependency} bias instance  where the model fails to locate the target entity in the mention (\textcolor{blue}{T9}) and two \emph{Overgeneralization} bias instances: \textcolor{blue}{T11} annotated by coarse types and \textcolor{blue}{T12} annotated by ultra-fine types. To quantify the overgeneralization bias (\Cref{sec:diagnosing_et_models}), we query the typing model with null input in \textcolor{red}{T13}. To mitigate spurious correlations (\Cref{sec:mitigating_spurious_correlations}), we do dependency parsing to distinguish headwords from dependents in \textcolor{green}{S6} and truncate the mention with only the headword preserved as \textcolor{green}{T10} to help address dependency bias.}
\label{tab:bias_example_II}
\end{table*}

In this section, we start with the problem definition (\Cref{sec:problem_definition}) and then categorize the spurious correlations %utilized by entity typing models between distinct textual features and entity types
causing shortcut predictions by the typing model (\Cref{sec:spurious_correlation_definition}). Next, we introduce our diagnosing strategy to identify biased predictions of entity typing models caused by such spurious correlations (\Cref{sec:diagnosing_et_models}). Lastly, we propose a counterfactual data augmentation approach to mitigate the identified spurious correlations, %and discuss alternative ways to adopt existing debiasing approaches to entity typing
as well as several alternative techniques that apply
(\Cref{sec:mitigating_spurious_correlations}).
\subsection{Problem Definition}\label{sec:problem_definition}
Given a sentence with $s$ an entity mention $e\in s$, the \emph{entity typing} task aims at predicting one or more words or phrases $T$ from the label space $L$ that describe the type(s) of $e$.

%o benefit the downstream context-sensitive tasks with identified entity types, we require that the selected entity type $T$ should be context sensitive. 
By nature, the inference of the type $T$ should be context-dependent.
Take the $1$st sample demonstrated in~\Cref{fig:spurious_correlations} as an instance: in ``Last week I stayed in \underline{\textbf{\emph{Treasure Island}}} for two nights when visiting Las Vegas,'' Treasure Island should be typed as ``hotel'' and ``resort'', rather than ``island'' or ``land'' by considering surface textual patterns underlying in the mention phrase.

% The definition of the label space $L$ varies across literature: some focused on predicting free-form words (e.g., place, hotel, etc)~\cite{ling2012fine,choi-etal-2018-ultra}, while the others aimed at predicting labels organized into a type hierarchy (e.g., /location/hotel) to allow domain knowledge incorporation and ensure label consistency~\cite{gillick2014context}. Considering the unclear hierarchy in the studied large-scale label space, we adopt the free-form types without ontologies in this work. Nevertheless, strategies to diagnose and mitigate spurious correlations proposed in this paper should apply to tasks on hierarchical label space as well.


\subsection{Defining Spurious Correlations}\label{sec:spurious_correlation_definition}
\nan{bias: table statistics+example; pronoun (unbalanced), lexical (simplicity), dependency (structure bias)}
\nan{Figure 1}
\nan{diagnosing: }
\nan{mitigating: approach for each bias}
\nan{correlation: model captures; data: shortcut features}
We systematically define six types of typical model biases caused by spurious correlations in entity typing models.

\muhao{\textbf{\emph{1) Mention-Context Bias}}:}
% Supervised learning models may rely overly on partial inputs without fully capturing the whole input content, e.g., predicting entailment determining whether a premise entails a hypothesis without seeing the premise sentence~\cite{gururangan-etal-2018-annotation,karimi-mahabadi-etal-2020-end}, leveraging claims without evidence for fact verification~\cite{schuster-etal-2019-towards,utama-etal-2020-mind,du2021towards}, etc. On the other hand,

%Entity typing is designed to infer mention types with reasoning on the full sentence to facilitate context-sensitive downstream tasks such as coreference resolution and question answering~\cite{choi-etal-2018-ultra}. However, we observe that existing models may \emph{overly rely on surface patterns of mentions to predict entity types}, which goes against the goal of such context-sensitive task.

Entity typing models normally address contexts and mentions separately, e.g., two bidirectional LSTMs to learn their respective representations in \emph{BiLSTM}~\cite{choi-etal-2018-ultra}, composing the input to the language model by separating the context and the mention with a special token $[sep]$ in \emph{MLMET}~\cite{dai-etal-2021-ultra}. 
% The mapping function from sentences and mention types and interactions among input features are majorly approximated by the last feed-forward layer. 
However, %training instances where the mention alone is sufficient for type prediction
semantically rich entity mentions %can be specifically meaningful, (e.g., mention \emph{India and other countries} and types \emph{area, region, state, country, location}, mention \emph{the war} and types \emph{battle, war, conflict}) 
may encourage the model to overly associate the mention surface with the type %during training, 
without considering the key information 
stated in contexts for some instances. We show an example \hyperlink{t1}{\textbf{T1}} and its perturbed counterpart \hyperlink{t2}{\textbf{T2}} in~\Cref{tab:bias_example_I}: making predictions considering the mention alone is misleading since the noun ``stuff'' and the name ``Janet'' look disconnected, hence the entity to type is unclear. Instead, ``Janet'' together with the right context ``recommended'' constitutes the adjective clause, which modifies the entity ``stuff'' to type. However, the model lacks the prior important reasoning process to  understand the interactions between the mention and the context, and infer types for the wrong entity ``Janet'' by giving the prediction \emph{person} whenever the full sentence or the mention is provided.

\textbf{\emph{2) Lexical Overlapping Bias}}:
%NLP models take advantage of high word-level overlaps between two components of task input, leading to poor generalization on samples requiring proper reasoning, e.g., hypothesis neither subsequence nor constituent of the premise but labeled with entailment~\cite{mccoy-etal-2019-right}, question pairs that are highly overlapping in words but majority labeled as non-duplicate in paraphrase identification~\cite{utama-etal-2020-mind}, etc.
Lexical overlapping between text pairs is an influential shortcut feature in entity typing. Specifically, \emph{mention words that have high lexical overlapping with entity types in the label set can normally describe the entity accurately}. Therefore, simply predicting the label word guarantees the high precision even without understanding mention.

As demonstrated in instance \hyperlink{t3}{\textbf{T3}} from~\Cref{tab:bias_example_I}: labeling mention ``next day'' with the single type ``day'' leads to $1.0$ precision and an f1 score as high as $0.749$ when additional type relevant to ``day'' are further inferred: \emph{time, date}. We observe a considerable amount of similar examples in the test set of \emph{UFET}, e.g., mention ``eye shields'' with label ``shield'', mention ``the Doha negotiations'' with label ``negotiation'', mention ``the standards for listing of that organization'' with label ``standard'', etc. 
Therefore, the highly overlapping in words between mention words and type labels make it difficult to evaluate whether the model makes predictions based on  content comprehension or simply according to lexical similarities.

\textbf{\emph{3) Named Entity Bias}}
% Training on convenient samples collected from news articles or social media, models are able to recognize named entities and utilize their popular senses for tasks such as named entity linking~\cite{goel-etal-2021-robustness} and named entity disambiguation~\cite{provatorova-etal-2021-robustness} with context cues ignored. 
% Models make predictions irrespective of the content by directly leveraging shortcuts between frequent named entities and annotated labels that co-occur frequently in the corpus.
To type mentions, models tend to \emph{link the contained named entities with its referred real-world objects and predict labels that co-occur frequently during training}, with contextual cues ignored. For instance, geopolitical areas such as \emph{India, London, Koscierzyna County} are normally labeled with types \emph{location, region, area}, organizations such as \emph{Budd Company, AARP Insurance Plan American Association, DirecTV} labeled with types \emph{organization, company, business, institution}, events such as \emph{World War I, the Battle of San Pasqual, the American Revolutionary War} labeled with types \emph{event, war, battle, conflict}, etc.

We show a concrete instance to type a person named entity in instance \hyperlink{t5}{\textbf{T5}} of~\Cref{tab:bias_example_I}. The mention \emph{Benjamin Netanyahu} is well-known for being the longest-serving Israeli prime minister in history. Occurring up to 107 times in \emph{UFET} entity linking training set, \emph{Benjamin Netanyahu} is normally annotated with \emph{politician, person, author, authority}. After observing the popular named entities and their common annotations during training, entity typing models are able to predict their representative tags precisely, with the F1 score as high as $1.0$ for the \emph{Benjamin Netanyahu} instance. With the shortcuts between popular named entities and their frequent labels, we can hardly evaluate models' capabilities to infer context-sensitive labels.

% For instance, entity typing models label the named entity mention in ``Bill Gates has donated billions to eradicate malaria,'' as businessman, since ``Bill Gates'' is well-known as the co-founder of the big tech company Microsoft. However, Gates should be typed as “philanthropist” based on his donation behavior discussed in the context.
\textbf{\emph{4) Pronoun Bias}}
Besides named entities and nominals, pronouns are one of the major noun mentions that typing models make predictions for~\cite{choi-etal-2018-ultra}. 
% However, common pronouns normally convey type information by themselves without referring to their contexts, e.g., mention ``he/him'' indicates types such as ``person'' and ``male'', while ``they'' implies types such as ``group''. Therefore, leveraging spurious correlations between pronouns and their common entity types observed in the training set can obtain reasonable and accurate predictions without reasoning on the role of the person or thing it plays in the context.
Pronouns could be much more frequent but much less diverse than real names of entities that have been mentioned before or currently talked about, e.g., the pronoun \emph{it} referring to a thing such as \emph{article, summit, New Zealand}, the pronoun \emph{we} indicating a group of people such as \emph{the police official, CCM health provider, SG investment company}, etc. Therefore, \emph{models are subject to biased training to type pronouns well, but lose the ability to type based on real names}.

To type the gender pronoun \emph{her} in the instance \hyperlink{t7}{\textbf{T7}} of \Cref{tab:bias_example_I}, the model successfully infer the indicated general types \emph{woman, female, person} and the context-sensitive type \emph{actress}. Overall, we expect models to infer types correctly for both pronoun entities and their indicated real names. 

\textbf{\emph{5) Dependency Bias}}
In dependency grammars, the syntactic structure of a sentence is described in terms of binary grammatical relations between headwords and dependent words that modify those heads~\cite{jurafsky2000speech}. For instance, in ``most car spoilers'', the dependent ``car'' is utilized to describe the position of the head object ``spoilers''.
It is observed that the mention's headwords explicitly match the mention to its types, and the adoption of distant supervision samples with headwords as mention types improved the typing model's accuracy~\cite{choi-etal-2018-ultra}. However, models may \emph{fail to capture the syntactic structure but make type predictions focusing on dependents instead of headwords}, especially when multiple noun phrases co-occur in the target mention. For the mention ``most car spoilers,'' the SOTA model \emph{MLMET} makes improper car-related predictions such as ``car'' and ``vehicle'', rather than inferring types of the headword ``spoilers''.

We show another instance with inappropriate focus on mention words in \hyperlink{t9}{\textbf{T9}} of~\Cref{tab:bias_example_II}: when the mention is composed of one concrete object ``whale'' as the dependent word and one abstract subject ``anatomy'' as the headword, the entity typing model fails to capture the crucial entity the context talks about, but gives ``whale''-related predictions such as \emph{animal}. Without recognizing the mention's syntactic structure, typing models make predictions irrelevant to the actual entity and result in extremely low accuracy.


\textbf{\emph{6) Overgeneralization Bias}}
When training models on imbalanced datasets with disproportional distributed labels, overgeneralization bias normally occurs, in which frequent labels are more likely to be predicted compared with rare ones. Entity typing datasets are also extremely imbalanced: coarse-grained labels, such as \emph{person, event} in dataset \emph{UFET}~\cite{choi-etal-2018-ultra} and \emph{/location, /other} in dataset \emph{OntoNotes}~\cite{gillick2014context}, cover the majority of samples and are more likely to be predicted compared with fine-grained but less frequent labels, e.g., \emph{pupil, comedy} in \emph{UFET} and \emph{/location/structure/sports\_facility, /other/heritage} in \emph{OntoNotes}.

We show two instances annotated by coarse- and fine-grained labels in \hyperlink{t11}{\textbf{T11}} and \hyperlink{t12}{\textbf{T12}} of~\Cref{tab:bias_example_II}: the model can easily predict the coarse-grained label \emph{person} (covering 824 out of 1998 training samples~\footnote{Statistical analyses on the crowd training set of \emph{UFET}. Note that although no instances are annotated by some ultra-fined labels such as \emph{abuse} or \emph{behavior}, models are trained on distant samples with these labels from entity linking and headword set.}) to describe \emph{anarchist}, but fail to infer less frequent labels such as \emph{misconduct} and \emph{wrongdoing} to type \emph{behavior}. Models ought to type entities according to reasoning on mentions and contexts, rather than follow the label distribution.

\paragraph{Discussion}
Since one instance may carry multiple kinds of biases, the prior defined six biases are not mutually exclusive. We discuss some possible (but not limited to) mixtures of concurrent biases as follows:
~\\$\bullet$ \emph{mention-context}, \emph{named entity} and \emph{overgeneralization} bias: in \hyperlink{t1}{T1} and \hyperlink{t2}{T2}, we show that the model overly relies on the mention to predict \emph{Janet}-relevant types without considering the context. We can explain this outcome from the perspective of: 1) \emph{named entity} bias: the model may recognize \emph{Janet} as a person named entity and predict the \emph{person} label since the two frequently co-occur in the training set ; 2) \emph{overgeneralization} bias: according to the statistics listed in~\Cref{tab:bias_example_II}, the coarse-grained type \emph{person} is popular among training samples and the model tends to predict frequent labels due to biased training. 
~\\$\bullet$ \emph{mention-context} and \emph{lexical overlapping} bias: the model falsely types the mention ``Treasure Island'' as \emph{island}, without understanding the context talking about the holiday accommodation. Another possible reason that the mention  far outweighs the context might be the high word similarity between the mention word ``Island'' and the type word ``island''. 
~\\$\bullet$ \emph{dependency} and \emph{lexical overlapping} bias: \emph{MLMET} incorrectly makes the prediction \emph{car}  for the mention ``most car spoilers'' without distinguishing important headwords from less important dependent words. Another reasonable explanation for emphasizing on the dependent rather than the headword is its perfect lexical match with the type set, where ``car'' is a relatively popular label but no type has high word similarity with ``spoilers''. 

To diagnose and mitigate all the spurious correlations the entity typing model may take advantage of, we will disentangle the multiple biases on a single instance by \textbf{analyzing each bias individually without considering their mutual interactions} in the following sections. 
% \muhao{(not needed in the arxiv version: do we have a way to estimate how frequent each type of biased cases may occur in existing datasets, and list those as a table? (perhaps can go to 3.2))}



\subsection{Diagnosing Entity Typing Models}\label{sec:diagnosing_et_models}
In previous section, we qualitatively inspect the existence of spurious correlations leveraged by a SOTA entity typing model %\emph{MLMET} 
on sampled instances with bias features. 
%However, to quantitatively measure the reliance of existing and future models on spurious correlations, we need to design a model-agnostic strategy to distinguish samples with bias features from those free of biases for a given testing set. 
To quantitatively measure the reliance of a model on spurious correlations
We hereby design model-agnostic strategy to distinguish samples causing biases to the model from those free of biases.

%Considering the world knowledge embedded in weights of models trained with massive amounts of data,
To do so, we propose to apply the PLM to zero-shot entity typing inference. 
Without further fine-tuning with task-centric objectives on entity typing datasets, %we believe
the PLM %achieve good performance on samples
is prompted to identify potentially biasing samples with
either detected surface patterns (e.g., \emph{mention-context} and \emph{lexical overlapping} bias) or facts (e.g., \emph{named entities} and \emph{pronoun} bias) captured during pre-training. %By analyzing zero-shot inference of PLMs, we are able to differentiate samples where predictive models may potentially exploit spurious correlations from those require sentence understanding and mention-context reasoning.
%Given biased features
Specifically, we reformulate entity typing as an entity type-specific cloze-style task and craft bias-based templates to prompt the PLM, \emph{RoBERTa}~\cite{liu2019roberta}, to fill in the blank.
The details are as follows.

\textbf{\emph{ Mention-Context Bias}}: Instead of providing the full sentence, we ask the language model to infer the entity type based only on the mention information with the following template:

\begin{tcolorbox}
\small
\quad$\mathbb{\bf Query}$: \emph{<Mention> is a type of <mask>.}
\end{tcolorbox}

As shown in \hyperlink{s1}{S1} from~\Cref{tab:bias_example_I}, \emph{RoBERTa} struggles to predict stuff-relevant types without any context, which is in consistent with the excessive attention of the well-trained entity typing model on the mention span reflected in \hyperlink{t1}{T1} and \hyperlink{t2}{T2}. 
In \hyperlink{s2}{S2}, on the contrary, \emph{RoBERTa} successfully infers all true types as well as two reasonable types of the mention ``the war'' without observing the context. Motivated by the noticable performance disparity achieved by the language model on distinct instances, we regard samples that the language model can accurately predict without the context information as biased. Entity typing models testing on these biased instances make it difficult to evaluate the model's capabilities to reason on sentences rather than leverage the spurious correlations between the mention and the entity labels.

\textbf{\emph{ Lexical Overlapping Bias}}:
To figure out whether the model makes correct predictions due to their highly lexical overlapping with the mention words, we substitute the sensitive word with a semantic similar but lexical different word and ask the language model to infer the entity type of such perturbed instance (we defer discussing perturbation details in~\Cref{sec:mitigating_spurious_correlations}). We adopt the following prompt template:

\begin{tcolorbox}
\small
\quad$\mathbb{\bf Query}$: \emph{<Left Context><New Mention with Word Substitution><Right Context>. <New Mention with Word Substitution> is a type of <mask>.}
\end{tcolorbox}

In \hyperlink{s3}{S3} of~\Cref{tab:bias_example_I}, we keep the original semantics of the mention and maintain the coherency of the new sentence by substituting ``day'' with ``twenty-four hour period''. Although such perturbation is insensible to humans, the language model rarely obtains any time-relevant types for the new mention, let alone the critical type ``day''. We consider instances with bias features that entity typing models may take advantage of, when the language model performs poorly after critical word substitution.

\textbf{\emph{ Named Entity Bias}}: To measure the knowledge learned about the named entities from prior training, we ask the language model to type the named entity when only the name and its general attribute is given, e.g., the geopolitical area \emph{India}, the organization \emph{Budd Company}, the event \emph{Word War I}, etc. We utilize the following template to construct the fill-in mask:

\begin{tcolorbox}
\small
\quad$\mathbb{\bf Query}$: \emph{The <Attribute> <Named Entity> is a type of <mask>.}
\end{tcolorbox}

In ~\Cref{tab:bias_example_I}, we show one instance with the mention contain the leader of the Opposition in Israel -- \emph{Benjamin Netanyahu}~\footnote{\url{https://en.wikipedia.org/wiki/Benjamin\_Netanyahu}} in \hyperlink{s4}{S4}, and Thai pop music singer -- \emph{Jintara Poonlarp}~\footnote{\url{https://en.wikipedia.org/wiki/Jintara\_Poonlarp}} in \hyperlink{s5}{S5}. Both of them are well-known people with their own biographical articles on Wikipedia, let alone thousands of news articles describing their past and latest updates. Since both the corpora for training language models and entity typing models are composed of Wikipedia articles and news reports, we believe the named entities that the PLM can accurately infer their types carry the prior knowledge bias, with which entity typing models tend to rely on the spurious correlations to make predictions.

\textbf{\emph{ Pronoun Bias}}: Compared with particular person names, gender pronouns show up much more frequently in articles to help make sentences smoother and clearer. To evaluate the model's real understanding of the referred person and their behavior according to the context, we substitute the gender pronoun with a random person name (we defer introducing substitution details in~\Cref{sec:mitigating_spurious_correlations}) and ask the language model to infer the person's type. Specifically, we utilize the following template as the prompt:

\begin{tcolorbox}
\small
\quad$\mathbb{\bf Query}$: \emph{<Left Context> <Person Name> <Right Context>. <Person Name> is a type of <mask>.}
\end{tcolorbox}

In \hyperlink{s6}{S6} of~\Cref{tab:bias_example_I}, we replace the popular pronoun mention \emph{her} with a random feminine given name \emph{Judith} and receive quite out-of-context type predictions from \emph{RoBERTa}. For instances with gender mentions, we consider them with pronoun bias when the language model fails to capture the majority of types after the name substitution. 

\textbf{\emph{ Overgeneralization Bias}}: To quantitatively measure the model's preference on popular types, we first craft a special instance -- an empty sentence, with which the uniform distribution over all types is expected from models free of overgeneralization bias. We then compute the divergence of the model's actual probability distribution: the higher/lower probability predicted on popular/rare types, the more biased the model on the label distribution. As shown in the instance \hyperlink{t13}{T13}, the studied entity typing model \emph{MLMET} gives the prediction \emph{person} with surprisingly high confidence, even though no actual entity is presented. We leave the analyses of probability distribution on both popular and rare types from more models in~\Cref{sec:exp}.

% Consider the \emph{named entity} bias example in \Cref{fig:spurious_correlations}, where Kevin Donovan is a filmmaker who has garnered international recognition with his commercials and music videos. 
% We first prompt RoBERTa~\cite{liu2019roberta} with ``\emph{The person Kevin Donovan is a type of <mask>}'' and then take the top type answers as the prediction, i.e., \{\emph{person, celebrity, character, personality, actor}\}. We consider this instance easy if the resulted f1 score can already go beyond a pre-defined threshold based on such a simple language model prompt. Accordingly, \textbf{we split %the samples with spurious correlations
% the identified simple cases
% into the \emph{easy} set, and those requiring proper reasoning into the \emph{hard} set.}
% Particularly, for \emph{overgeneralization} bias, we simply extract samples labeled only with coarse grained types into the easy split while those labeled with ultra-fine grained types into the hard split.


% Then we convert the easy instances to new instances where entity typing models are less prone to exploit spurious correlations: 1) \emph{mention-context} bias: query the model with mention alone; 2) \emph{lexical overlapping} bias: extract synsets of mention words that share the same lemmas as entity labels and substitute them by synonyms with semantics preserved; 3) \emph{named entity} bias: replacing named entities in easy instances with those recognized as the same named entity category but from hard instances; 4) \emph{pronoun} bias: replace gender pronouns with the actual person's name it refers to if exists, or random masculine/feminine names otherwise; 5) \emph{dependency} bias: keep the headwords in mentions to allow models make predictions given contexts and explicit headwords; 6) \emph{overgeneralization} bias: feed models with empty input to investigate the divergence of predicted label probabilities from the expected uniform distribution. For instance, to get rid of named entity bias, Brennan, recognized as the same named entity type ``person'' as Kevin Donovan but from another hard instance, is used as a replacement, as shown in Fig.~\Cref{fig:spurious_correlations}. Thereafter, the model cannot make accurate predictions as before even the context is unchanged and sufficient enough to infer the entity types. 


\subsection{Mitigating Spurious Correlations}\label{sec:mitigating_spurious_correlations}
\muhao{This part needs to focus on technical details of counterfactual data augmentation.}
After training on instances with bias features, models tend to leverage spurious correlations between shortcut features and entity labels and may achieve good performance on the testing instances sampled from the same distribution as the training set. However, models exploiting spurious correlations lack the required reasoning capability, and inevitably obtain poor out-of-distribution generalization when bias features observed during training do not hold.

To improve generalization, we propose to mitigate spurious correlations learned during training with a counterfactual data augmentation way: for each instance recognized with specific bias features, we automatically craft their bias-free counterpart and retrain entity typing models with both samples. Whenever the model learns to exploit spurious correlations on original training instances with bias features,  it will fail on newly crafted bias-free instances and actively look for a robust strategy leading to double-win: understand and reason on sentences rather than exploit spurious correlations. 
Considering the characteristic textual patterns from different biases, we propose the following distinct strategies to craft new instances free from each bias:

\textbf{\emph{Lexical Overlapping Bias}} we perform word substitutions in two steps to remove mention words lexically similar to type labels with original semantics preserved: \emph{1) candidate word selection}: from WordNet~\cite{miller1995wordnet}, search for non-type word synonyms of different senses (i.e., defined as ``synset'' in WordNet that contains a set of synonyms that share a common meaning), \emph{2) sematic meaning preservation}: distinguish the word sense in the original sentence and pick the synonyms from the correct synset. 

We consider the following sentence as an instance: ``Deutsche Bank would neither confirm nor deny the \underline{\textbf{\emph{discharge}}} of the two executives, and it also would not specify who was the target of the alleged spying'', annotated with types \emph{dismissal, discharge, leave, termination}. Since ``discharge'' shows up both in the mention and the true labels, we perform word substitutions with synonym candidates from 20 synsets found in WordNet. We show a few synsets with popular senses as follows:

\quad$\mathbb{\bf Synset}$ I: (\emph{the termination of someone's employment}) dismissal, dismission, discharge, firing, liberation, release, sack, sacking

\quad$\mathbb{\bf Synset II}$: (\emph{a substance that is emitted or released}) discharge, emission

\quad$\mathbb{\bf Synset III}$: (\emph{a formal written statement of relinquishment}) release, waiver, discharge

Synonyms that share high word similarities with the true labels are removed to avoid creating new lexical overlapping bias features, e.g., \emph{dismissal, discharge} from Synset I, \emph{discharge} from Synset II and Synset III. To guarantee the semantic consistency of the new sentence and the fidelity of true labels to type the new mention, we leverage available word sense disambiguation models to preserve synonyms from the synset that is most consistent with the sense used in the original sentence: \emph{dismission, firing, liberation, release, sack, sacking} from Synset I are finally selected to substitute ``discharge''. We consider perturbed sentences with poor performance from the language model (e.g., ``day'' substituted by ``twenty-four hour period'' in \hyperlink{s3}{S3}) as the \textbf{hard set} free from lexical overlapping bias, to prohibit the entity typing model from exploiting spurious correlations. As shown in \hyperlink{t4}{T4}, without training on the bias-free hard set, \emph{MLMET} no longer predicts the critical word ``day'', but some surface word ``period'' instead.

\textbf{\emph{Named Entity Bias}} To disentangle memorizing well-known attributes of named entities from inferring their actual types based on sentence understanding, we perform named entity substitution with both the validity and bias-free criteria: \emph{1) validity}: new named entities should stand for the real objects with the same attribute, e.g., the geopolitical area ``India'' replace by  ``London'', the organization ``Budd Company'' replaced by ``AARP Insurance Plan American Association'', the event ``World War I'' replaced by ``the Battle of San Pasqual'', etc; \emph{2) bias-free}: models training on large corpora should not possess prior knowledge about the new named entities so that capabilities on sentence understanding could be well tested. Basically, we leverage available named entity recognition models to identify and classify named entities 
into general attribute types, and then divide them into \textbf{informative} and \textbf{non-informative} group according to typing performance from the language model. We then substitute ``informative'' named entities with ``non-informative'' ones sharing the same attribute and train entity typing models on the newly crafted \textbf{hard} instances.

Compared with the politician \emph{Benjamin Netanyahu}, the language model can hardly infer the impression of the single \emph{Jintara Poonlarp} on the public. Particularly, only general types to describe person named entities are predicted in \hyperlink{s5}{S5}: \emph{person, human, woman}. We then consider \emph{Benjamin Netanyahu} as an ``easy'' named entity containing much prior knowledge, while \emph{Jintara Poonlarp} as an ``hard'' named entity without much type-relevant information revealed. After substituting \emph{Benjamin Netanyahu} with \emph{Jintara Poonlarp} in \hyperlink{t6}{T6}, \emph{MLMET} can hardly infer the political role the new mention by analyzing its connection with the politician (\emph{Amin al-Husseini}, Palestinian Arab nationalist and Muslim leader in Mandatory Palestine~\footnote{\url{https://en.wikipedia.org/wiki/Amin\_al-Husseini}}) and political description (``masterminds'' and ``Holocaust'') in the context. \emph{MLMET} even crashes with some out-of-context predictions: \emph{scholar, writer}.

\textbf{\emph{Pronoun Bias}} Pronouns are widely utilized to refer to a noun used earlier in the passage. In an entity typing sentence, the pronoun mention should refer to the entity in either the given context or the absent context. Accordingly, we craft \textbf{hard} instances by concretizing gender pronoun mentions from two perspectives: \emph{1) the referred item in the given context}: we first adopt available coreference resolution models to search for the expression that refers to the same entity as the pronoun, e.g., the mention ``he'' refers to
``Clarke'' in the sentence ``While Clarke was responsible for most of the punishment ( \underline{\textbf{\emph{he}}} made six birdies , one matching a Woods birdie at the eighth , one matching a Duval birdie at the ninth , and that winning birdie at 17 ) , the Americans never made things happen''; \emph{2) the referred item in the absent context}: for pronouns without coreference expression, we substitute the gender pronoun with a randomly sampled masculine/feminine name from the corpus, e.g., \emph{Lorelle, Daphne, Edithe, Carrissa, Keely} for \emph{she}/\emph{her}, \emph{Oleg, Meyer, Alexander, Stanly, Torre} for \emph{he}/\emph{him}/\emph{his}. New sentences with the actual person names as mentions are considered \textbf{hard} if the language model fails to infer the person's type with contextual information given.

As shown in the original instance \hyperlink{t7}{T7} of~\Cref{tab:bias_example_I}, the actual person's name that the pronoun mention ``Her'' refers to is not  provided in the current sentence. As a result, a random feminine name, ``Judith'' is assumed to be the referred entity and substitutes the pronoun mention as a new sentence in \hyperlink{s6}{S6}. Considering the ridiculously wrong types predicted by \emph{RoBERTa} such as \emph{bird} and \emph{cat}, we include this new instance in the hard set and expect the entity modeling training on this kind of pronoun bias-free instances to infer person name types as accurate as pronoun types. Beforehand, we test on the new crafted instance without counterfactual augmented training, and observe huge performance drop after pronoun concretization: types related to the name's gender attribute such as \emph{woman} and \emph{female} are missing, let alone the types requiring fully context understanding such as \emph{actress}. 

\textbf{\emph{Dependency Bias}}: To encourage the model to type for the correct target entity, we augment the original instance within two steps: \emph{1) dependency parsing}: we leverage available dependency parsing tools to recognize grammatical relations between the words, e.g., \emph{(most, spoilers), (car, spoilers), (spoilers, spoilers)} are dependents and their respective head words in the mention ``most car spoilers''; \emph{2) mention truncation}: given the observation that the headword is most likely to be the target entity to type, we truncate all other dependent words in the new mention as the \textbf{hard} instance, e.g., ``most car spoilers'' substituted by ``spoilers''.

For instance \hyperlink{t9}{T9} in~\Cref{tab:bias_example_I}, we show their mention word dependency analysis in \hyperlink{s6}{S6} and predictions on the perturbed instance in \hyperlink{t10}{T10}. Without distractions from other dependent words in the new mention, \emph{MLMET} spares no effort to infer types of the target entity ``whale'' with the correct prediction \emph{subject}. Motivated by the improved performance when the mention headword is specifically provided, we believe entity typing models can actively learn to capture target entity among mention words when both original sentences and their hard counterparts are given during training. In such augmented training regime, the entity typing model is expected achieve robust performance on new sentences bearing distractions from dependent words in mentions.

\paragraph{Evaluating Debiasing Approaches on Identified Biases} In \emph{AFLite}~\cite{le2020adversarial}, it is assumed that NLP models may utilize spurious correlations in samples with which simple models such as fasttext~\cite{joulin-etal-2017-bag} can predict accurately. Therefore, we adopt \emph{AFLite} by dropping these easy samples and training entity typing models with remaining hard ones only.

Another popular direction to mitigate spurious correlations compares model outputs given full input and biased input. According to our defined biases and diagnosing strategy, we extract bias features (partial input such as the \emph{mention}, the \emph{named entities}, the \emph{pronoun}, the \emph{NULL} input) and compare our counterfactual augmented training with the following debiasing approaches: 
\emph{1) ensemble-based bias mitigation approaches}: they are composed of one bias model that learns  from bias features alone and another base model that is trained to focus less on samples predicted corrected by the bias model. Typical approaches include product of experts~\cite{clark-etal-2019-dont,he-etal-2019-unlearn,karimi-mahabadi-etal-2020-end}, debiased focal loss~\cite{karimi-mahabadi-etal-2020-end}, learned-mixin and its variant learned-mixin+H~\cite{clark-etal-2019-dont}; \emph{2) contrastive learning}~\cite{chen2021exploring}: the contrastive loss is utilized to discourage the model from learning similar representations for full features and bias features. The loss function can be formulated based on the cross entropy~\cite{caron2021emerging} or the cosine similarity~\cite{chen2021exploring}; \emph{3) counterfactual inference}~\cite{qian-etal-2021-counterfactual}: the influence of spurious correlations on predictions is mitigated by deducting the model's logits given the full input with logits given bias features.

==> diagnosing.tex <==
\section{Diagnosing Entity Typing Models}
\subsection{Mention-context Bias}
\begin{table}[h!]
\begin{tabular}{@{}lcccc@{}}
\toprule
model     & \begin{tabular}[c]{@{}c@{}}easy-f1 \\ (m-c)\end{tabular} & \begin{tabular}[c]{@{}c@{}}easy-f1 \\ (m)\end{tabular}    & \begin{tabular}[c]{@{}c@{}}hard-f1 \\ (m-c)\end{tabular} & \begin{tabular}[c]{@{}c@{}}hard-f1 \\ (m)\end{tabular}     \\ \midrule
bilstm    & 0.385                                                    & \begin{tabular}[c]{@{}c@{}}0.400 \\ (3.8\%)\end{tabular}  & 0.265                                                    & \begin{tabular}[c]{@{}c@{}}0.253 \\ (-4.7\%)\end{tabular}  \\\midrule
labelgcn  & 0.521                                                    & \begin{tabular}[c]{@{}c@{}}0.507 \\ (-2.6\%)\end{tabular} & 0.317                                                    & \begin{tabular}[c]{@{}c@{}}0.298 \\ (-5.8\%)\end{tabular}  \\\midrule
box4types & 0.586                                                    & \begin{tabular}[c]{@{}c@{}}0.554 \\ (-5.5\%)\end{tabular} & 0.380                                                    & \begin{tabular}[c]{@{}c@{}}0.343 \\ (-9.8\%)\end{tabular}  \\\midrule
lrn       & 0.519                                                    & \begin{tabular}[c]{@{}c@{}}0.522 \\ (0.5\%)\end{tabular}  & 0.367                                                    & \begin{tabular}[c]{@{}c@{}}0.319 \\ (-13.1\%)\end{tabular} \\\midrule
mlmet     & 0.654                                                    & \begin{tabular}[c]{@{}c@{}}0.654 \\ (0.0\%)\end{tabular}  & 0.436                                                    & \begin{tabular}[c]{@{}c@{}}0.395 \\ (-9.4\%)\end{tabular}  \\ \bottomrule
\end{tabular}
\caption{\label{tab:mention_context_bias}\textbf{Mention-context} Bias. Easy samples: 131, hard samples: 1085. \emph{m-c} means predicting normally (with mention-context), while \emph{m} means predicting with mention alone. \textcolor{red}{\emph{1st vs. 2nd} column}: models obtain similar performance without context information; \textcolor{red}{\emph{3rd vs. 4th} column}: model obtain better performance when given context information; \textcolor{red}{\emph{1st vs 3rd} column}: models obtain better performance when mention is more informative than context.}
\end{table}
\subsection{Lexical Overlapping Bias}
\begin{table}[h!]
\begin{tabular}{@{}lcccc@{}}
\toprule
model     & \begin{tabular}[c]{@{}c@{}}easy-f1 \\ (origin)\end{tabular} & \begin{tabular}[c]{@{}c@{}}easy-f1 \\ (syn.)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}hard-f1 \\ (origin)\end{tabular} & \begin{tabular}[c]{@{}c@{}}hard-f1 \\ (syn.)\end{tabular}  \\ \midrule
bilstm    & 0.392                                                       & \begin{tabular}[c]{@{}c@{}}0.167 \\ (-57.5\%)\end{tabular} & 0.510                                                       & \begin{tabular}[c]{@{}c@{}}0.050 \\ (-90.3\%)\end{tabular} \\\midrule
labelgcn  & 0.414                                                       & \begin{tabular}[c]{@{}c@{}}0.111 \\ (-73.1\%)\end{tabular} & 0.403                                                       & \begin{tabular}[c]{@{}c@{}}0.162 \\ (-59.9\%)\end{tabular} \\\midrule
box4types & 0.267                                                       & \begin{tabular}[c]{@{}c@{}}0.333 \\ (25.0\%)\end{tabular}  & 0.186                                                       & \begin{tabular}[c]{@{}c@{}}0.115 \\ (-38.3\%)\end{tabular} \\\midrule
lrn       & 0.111                                                       & \begin{tabular}[c]{@{}c@{}}0.095 \\ (-14.3\%)\end{tabular} & 0.133                                                       & \begin{tabular}[c]{@{}c@{}}0.093 \\ (-29.7\%)\end{tabular} \\\midrule
mlmet     & 0.544                                                       & \begin{tabular}[c]{@{}c@{}}0.444 \\ (-18.2\%)\end{tabular} & 0.551                                                       & \begin{tabular}[c]{@{}c@{}}0.327 \\ (-40.8\%)\end{tabular} \\ \bottomrule
\end{tabular}
\caption{\label{tab:lexical_overlapping_bias}\textbf{Lexical Overlapping} Bias. Easy samples: 3, hard samples: 475. \emph{origin} means predicting with regular input (at least one gold label shows up in mention), while \emph{syn.} means predicting with gold labels in mention replaced by their synonyms. \textcolor{red}{\emph{1st vs. 2nd} and \emph{3rd vs. 4th} column}: performance drops after replacing label hints in mention by different words with semantics preserved. \textcolor{red}{\emph{2nd vs 4th} column}: obvious performance drop on majority of samples.}
\end{table}
\subsection{Named Entity Bias}
\begin{table*}[h!]
\begin{tabular}{@{}lcccccc@{}}
\toprule
model     & \begin{tabular}[c]{@{}c@{}}easy-f1 \\ (full)\end{tabular} & \begin{tabular}[c]{@{}c@{}}easy-f1 \\ (ne)\end{tabular} & \begin{tabular}[c]{@{}c@{}}easy-f1 \\ (aug hard)\end{tabular} & \begin{tabular}[c]{@{}c@{}}hard-f1 \\ (full)\end{tabular} & \begin{tabular}[c]{@{}c@{}}hard-f1 \\ (ne)\end{tabular} & \begin{tabular}[c]{@{}c@{}}hard-f1 \\ (aug easy)\end{tabular} \\ \midrule
bilstm    & 0.504                                                     & 0.473 (-6.0\%)                                          & 0.332 (-34.0\%)                                               & 0.316                                                     & 0.201 (-36.4\%)                                         & 0.372 (17.6\%)                                                \\
labelgcn  & 0.610                                                     & 0.585 (-4.1\%)                                          & 0.442 (-27.5\%)                                               & 0.376                                                     & 0.234 (-37.6\%)                                         & 0.444 (18.2\%)                                                \\
box4types & 0.671                                                     & 0.647 (-3.7\%)                                          & 0.508 (-24.4\%)                                               & 0.457                                                     & 0.264 (-42.3\%)                                         & 0.503 (10.2\%)                                                \\
lrn       & 0.641                                                     & 0.645 (0.7\%)                                           & 0.525 (-18.0\%)                                               & 0.453                                                     & 0.259 (-42.9\%)                                         & 0.513 (13.4\%)                                                \\
mlmet     & 0.735                                                     & 0.705 (-4.1\%)                                          & 0.600 (-18.4\%)                                               & 0.505                                                     & 0.291 (-42.2\%)                                         & 0.539 (6.9\%)                                                 \\ \bottomrule
\end{tabular}
\caption{\label{tab:named_entity_bias}\textbf{Named Entity} Bias. Easy samples: 36, hard samples: 500. \emph{full} means predicting with context and mention including named entities, \emph{ne} means predicting with context and named entities, \emph{aug hard} means predicting with context and named entities of the same group (i.e., company Apple and Microsoft) but from the opposite hard level, i.e., easy$\rightarrow$hard and hard$\rightarrow$easy. \textcolor{red}{\emph{1st vs. 2nd} column}: model performance maintains when the connection between named entity group and mention label is easy to captured; \textcolor{red}{\emph{4th vs. 5th} column}: model performance drops a lot when the connection between named entity group and mention label is hard to captured; \textcolor{red}{\emph{1st vs. 3rd} column}: model performance drops after replacing named entities by those easy to detect its attribute and connection with mention label; \textcolor{red}{\emph{4th vs 6th} column}: model performance improves after replacing named entities by those hard to detect its attribute and connection with mention label.}
\end{table*}
\subsection{Gender Pronoun Bias}
\begin{table}[h!]
\begin{tabular}{@{}lcccc@{}}
\toprule
model     & \begin{tabular}[c]{@{}c@{}}easy-f1 \\ (p-c)\end{tabular} & \begin{tabular}[c]{@{}c@{}}easy-f1 \\ (n-c)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}hard-f1 \\ (p-c)\end{tabular} & \begin{tabular}[c]{@{}c@{}}hard-f1 \\ (n-c)\end{tabular}   \\ \midrule
bilstm    & 0.366                                                    & \begin{tabular}[c]{@{}c@{}}0.130 \\ (-64.6\%)\end{tabular} & 0.494                                                    & \begin{tabular}[c]{@{}c@{}}0.179 \\ (-63.8\%)\end{tabular} \\\midrule
labelgcn  & 0.575                                                    & \begin{tabular}[c]{@{}c@{}}0.378 \\ (-34.4\%)\end{tabular} & 0.511                                                    & \begin{tabular}[c]{@{}c@{}}0.395 \\ (-22.8\%)\end{tabular} \\\midrule
box4types & 0.736                                                    & \begin{tabular}[c]{@{}c@{}}0.603 \\ (-18.1\%)\end{tabular} & 0.565                                                    & \begin{tabular}[c]{@{}c@{}}0.435 \\ (-23.0\%)\end{tabular} \\\midrule
lrn       & 0.448                                                    & \begin{tabular}[c]{@{}c@{}}0.421 \\ (-6.0\%)\end{tabular}  & 0.570                                                    & \begin{tabular}[c]{@{}c@{}}0.541 \\ (-5.2\%)\end{tabular}  \\\midrule
mlmet     & 0.683                                                    & \begin{tabular}[c]{@{}c@{}}0.659 \\ (-3.5\%)\end{tabular}  & 0.561                                                    & \begin{tabular}[c]{@{}c@{}}0.525 \\ (-6.4\%)\end{tabular}  \\ \bottomrule
\end{tabular}
\caption{\label{tab:pronoun_bias}\textbf{Pronoun} Bias. Easy samples: 20, hard samples: 881.}
\end{table}
\subsection{Dependency Bias}
\begin{table}[h!]
\begin{tabular}{@{}lccc@{}}
\toprule
model     & \#increase & \begin{tabular}[c]{@{}c@{}}f1 \\ (m-c)\end{tabular} & \begin{tabular}[c]{@{}c@{}}f1 \\ (h-c)\end{tabular} \\ \midrule
bilstm    & 280/961    & 0.152                                               & 0.396 (160.5\%)                                     \\
labelgcn  & 238/961    & 0.321                                               & 0.517 (61.2\%)                                      \\
box4types & 149/961    & 0.399                                               & 0.574 (43.9\%)                                      \\
lrn       & 128/961    & 0.372                                               & 0.549 (47.4\%)                                      \\
mlmet     & 222/961    & 0.424                                               & 0.564 (32.9\%)                                      \\ \bottomrule
\end{tabular}
\caption{\label{tab:dependency_bias}\textbf{Dependency} Bias.}
\end{table}
\subsection{Overgeneralization}
\begin{table*}[h!]
\begin{tabular}{@{}lccl@{}}
\toprule
model     & \begin{tabular}[c]{@{}c@{}}easy\\ (f1)\end{tabular} & \begin{tabular}[c]{@{}c@{}}hard\\ (f1)\end{tabular} & \multicolumn{1}{c}{top/tail type (prob)}                                                                                                                                                           \\ \midrule
bilstm    & 0.466                                               & 0.118                                               & \begin{tabular}[c]{@{}l@{}}person (.928), title (.437), concept (.104), communicator (.062)...\\ ...headman (.000), vice squad (.000), adolescent (.000), supporter (.000)\end{tabular}            \\\midrule
labelgcn  & 0.465                                               & 0.152                                               & \begin{tabular}[c]{@{}l@{}}concept (.349), increase (.249), case (.192), idea (.158)...\\ ...data structure (.000), archipelago (.000), spiritual leader (.000), national park (.000)\end{tabular} \\\midrule
box4types & 0.454                                               & 0.132                                               & \begin{tabular}[c]{@{}l@{}}object (.626), person (.282), company (.231), product (.220)...\\ ...horrible (.000), dismissal (.000), trump (.000), small town (.000)\end{tabular}                    \\\midrule
lrn       & 0.554                                               & 0.116                                               & \begin{tabular}[c]{@{}l@{}}person (.998), writer (.000), place (.000), male (.000)...\\ ...chicken feed (.000), chicken leg (.000), chicken wing (.000), chicken wire (.000)\end{tabular}          \\\midrule
mlmet     & 0.427                                               & 0.232                                               & \begin{tabular}[c]{@{}l@{}}person (.992), time (.314), title (.100), place (.017)...\\ ...military service (.000), consortium (.000), negotiator (.000), football player (.000)\end{tabular}       \\ \bottomrule
\end{tabular}
\caption{\label{tab:overgeneralization_bias}\textbf{Overgeneralization} Bias. Easy samples: 93, had samples:242.}
\end{table*}
